Online Learning Based Mobile Robot Controller Adaptation for Slip Reduction

Slip is a very common phenomena present in wheeled mobile robotic systems. It has undesirable consequences such as wasting energy and impeding system stability. To tackle the challenge of mobile robot trajectory tracking under slippery conditions, we propose a hierarchical framework that learns and adapts gains of the tracking controllers simultaneously online. Concretely, a reinforcement learning (RL) module is used to auto-tune parameters in a lateral predictive controller and a longitudinal speed PID controller. Experiments show the necessity of simultaneous gain tuning, and have demonstrated that our online framework outperforms the best baseline controller using fixed gains. By utilizing online gain adaptation, our framework achieves robust tracking performance by rejecting slip and reducing tracking errors when the mobile robot travels through various terrains.

==> related_work.tex <==

% \subsection{Trajectory tracking under slippery conditions
% }

% To mitigate slipping, many works try to identify slip parameters or terrain states, and design simple control laws with robot kinematic models, e.g. \cite{burke2012path,pico2022climbing,kim2016kinematic}.  \cite{sebastian2019active, wang2020trajectory} further choose to model slip as disturbance in the kinematics model using observers. However, state vectors are of high order and matrix inverse calculations could be massive.


% Another line of work focuses on wheel dynamics with traction forces. \cite{tian2009modeling} choose to use Magic formula to derive the relationship between traction force and slip ratio, while \cite{nandy2011detailed} formulates a detailed slip dynamics with certain switching conditions. Although dynamic models consider forces in addition to kinematics models, they usually require system identification for different scenarios and have poor generalization abilities. 

% There are also other works utilizing reinforcement learning to directly learn a policy, such as in \cite{xu2018zero, cai2020high}. But end-to-end RL approaches require considerable training time and poses challenges in explainability. Instead of end-to-end RL, \cite{carlucho2019double} only uses RL to optimize controllers, but the results are highly dependent on action space discretization. Our work follows a similar approach. We use 

% \subsection{Online gain tuning}
% Many works on using machine learning and reinforcement learning algorithms to optimize PID parameters. 

% \cite{nyberg2017optimizing}: Evolutionary programming (EP) method for optimizing PID parameters.

% \cite{han2017lateral}
% \cite{carlucho2019double} double Q-Learning algorithm for fast on-line adaptation of multiple low-level PID controllers. but if the discretization is coarse the results could be poor, on the other hand, if it is too thin the Q-learning algorithm could become intractable. Also full PID many variables, hard to learn and sometimes not necessary.






